ToDo: Token Downsampling for Efficient Generation of High-Resolution Images

Attention mechanism has been crucial for image diffusion models, however, their quadratic computational complexity limits the sizes of images we can process within reasonable time and memory constraints. This paper investigates the importance of dense attention in generative image models, which often contain redundant features, making them suitable for sparser attention mechanisms. We propose a novel training-free method ToDo that relies on token downsampling of key and value tokens to accelerate Stable Diffusion inference by up to 2x for common sizes and up to 4.5x or more for high resolutions like 2048x2048. We demonstrate that our approach outperforms previous methods in balancing efficient throughput and fidelity.

==> images/Lowest_Sim_3x3_V1.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
title={Lowest similarity in 3x3 neighborhood 1024x1024},
x grid style={darkgray176},
xlabel={Timesteps},
xmin=8.5, xmax=41.5,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Similarity},
ymin=0.66294007660905, ymax=0.957558957640234,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
10 0.944167190320635
25 0.850567606842883
40 0.792913009894322
};
\addlegendentry{depth 0 down}
\addplot [semithick, darkorange25512714]
table {%
10 0.918062291903056
25 0.799066615570015
40 0.750836928225311
};
\addlegendentry{depth 0 up}
\addplot [semithick, forestgreen4416044]
table {%
10 0.878891205533291
25 0.718125754588082
40 0.676331843928649
};
\addlegendentry{depth 1 down}
\addplot [semithick, crimson2143940]
table {%
10 0.934043507180759
25 0.860763206258925
40 0.811068555889651
};
\addlegendentry{depth 1 up}
\end{axis}

\end{tikzpicture}

==> images/TestTikz.tex <==
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
title={lowest similarity value in a 5x5 neighborhood 1024x1024},
x grid style={darkgray176},
xlabel={Timesteps},
xmin=8.5, xmax=41.5,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Similarity},
ymin=0.511386021927678, ymax=0.883726277284478,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
10 0.866801720222805
25 0.72087160140416
40 0.639920758909815
};
\addlegendentry{depth 0 down}
\addplot [semithick, darkorange25512714]
table {%
10 0.807462904701012
25 0.62138479282081
40 0.563029844519977
};
\addlegendentry{depth 0 up}
\addplot [semithick, forestgreen4416044]
table {%
10 0.779273922311404
25 0.57685960675183
40 0.528310578989351
};
\addlegendentry{depth 1 down}
\addplot [semithick, crimson2143940]
table {%
10 0.855059663881839
25 0.730848003892043
40 0.639925151378937
};
\addlegendentry{depth 1 up}
\end{axis}

\end{tikzpicture}

==> images/graph_perf_text_sq.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.1,0.5,0.7}
\definecolor{color1}{rgb}{0.907843137254902,0.487254901960784,0.354901960784314}
\definecolor{color2}{rgb}{0.258333333333333,0.678921568627451,0.59656862745098}
\definecolor{color3}{rgb}{0.917647058823529,0.638235294117647,0.423529411764706}
\definecolor{color4}{rgb}{0.208333333333333,0.387745098039216,0.423039215686274}

\begin{axis}[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black,
  fill=white!89.8039215686275!black
},
tick align=outside,
tick pos=left,
title={Performance Comparison Across Resolutions},
x grid style={white!82.7450980392157!black},
xlabel={Resolution},
xmajorgrids,
xmin=-0.5, xmax=2.5,
xtick style={color=white!33.3333333333333!black},
xtick={0,1,2},
xticklabels={1024,1536,2048},
y grid style={white!82.7450980392157!black},
ylabel={Relative Performance Increase Against Baseline},
ymajorgrids,
ymin=0, ymax=4.61736926438456,
ytick style={color=white!33.3333333333333!black}
]
\draw[draw=none,fill=color0,fill opacity=0.9,line width=0.32pt] (axis cs:-0.46,0) rectangle (axis cs:-0.276,1);
\draw[draw=none,fill=color0,fill opacity=0.9,line width=0.32pt] (axis cs:0.54,0) rectangle (axis cs:0.724,1);
\draw[draw=none,fill=color0,fill opacity=0.9,line width=0.32pt] (axis cs:1.54,0) rectangle (axis cs:1.724,1);
\draw[draw=none,fill=color1,fill opacity=0.9,line width=0.32pt] (axis cs:-0.276,0) rectangle (axis cs:-0.0919999999999999,1.60083499727718);
\draw[draw=none,fill=color1,fill opacity=0.9,line width=0.32pt] (axis cs:0.724,0) rectangle (axis cs:0.908,2.94993429697766);
\draw[draw=none,fill=color1,fill opacity=0.9,line width=0.32pt] (axis cs:1.724,0) rectangle (axis cs:1.908,4.29525923396506);
\draw[draw=none,fill=color2,fill opacity=0.9,line width=0.32pt] (axis cs:-0.092,0) rectangle (axis cs:0.092,1.59677711388738);
\draw[draw=none,fill=color2,fill opacity=0.9,line width=0.32pt] (axis cs:0.908,0) rectangle (axis cs:1.092,2.94548317260382);
\draw[draw=none,fill=color2,fill opacity=0.9,line width=0.32pt] (axis cs:1.908,0) rectangle (axis cs:2.092,4.28100626790323);
\draw[draw=none,fill=color3,fill opacity=0.9,line width=0.32pt] (axis cs:0.0920000000000001,0) rectangle (axis cs:0.276,1.51737783895389);
\draw[draw=none,fill=color3,fill opacity=0.9,line width=0.32pt] (axis cs:1.092,0) rectangle (axis cs:1.276,2.43693009118541);
\draw[draw=none,fill=color3,fill opacity=0.9,line width=0.32pt] (axis cs:2.092,0) rectangle (axis cs:2.276,3.1744269190326);
\draw[draw=none,fill=color4,fill opacity=0.9,line width=0.32pt] (axis cs:0.276,0) rectangle (axis cs:0.46,1.66176747691728);
\draw[draw=none,fill=color4,fill opacity=0.9,line width=0.32pt] (axis cs:1.276,0) rectangle (axis cs:1.46,3.04372584909498);
\draw[draw=none,fill=color4,fill opacity=0.9,line width=0.32pt] (axis cs:2.276,0) rectangle (axis cs:2.46,4.3974945375091);
\draw[draw=none,fill=color0,fill opacity=0.9,line width=0.32pt] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0,fill opacity=0.9,line width=0.32pt};
\addlegendentry{Baseline}

\draw[draw=none,fill=color1,fill opacity=0.9,line width=0.32pt] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1,fill opacity=0.9,line width=0.32pt};
\addlegendentry{ToMe (0.75)}

\draw[draw=none,fill=color2,fill opacity=0.9,line width=0.32pt] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=color2,fill opacity=0.9,line width=0.32pt};
\addlegendentry{ToMe (0.89)}

\draw[draw=none,fill=color3,fill opacity=0.9,line width=0.32pt] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=color3,fill opacity=0.9,line width=0.32pt};
\addlegendentry{ToDo (0.75)}

\draw[draw=none,fill=color4,fill opacity=0.9,line width=0.32pt] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=color4,fill opacity=0.9,line width=0.32pt};
\addlegendentry{ToDo (0.89)}

\addplot [line width=0.72pt, white!26!black, forget plot]
table {%
-0.368 nan
-0.368 nan
};
\addplot [line width=0.72pt, white!26!black, forget plot]
table {%
0.632 nan
0.632 nan
};
\addplot [line width=0.72pt, white!26!black, forget plot]
table {%
1.632 nan
1.632 nan
};
\addplot [line width=0.72pt, white!26!black, forget plot]
table {%
-0.184 nan
-0.184 nan
};
\addplot [line width=0.72pt, white!26!black, forget plot]
table {%
0.816 nan
0.816 nan
};
\addplot [line width=0.72pt, white!26!black, forget plot]
table {%
1.816 nan
1.816 nan
};
\addplot [line width=0.72pt, white!26!black, forget plot]
table {%
0 nan
0 nan
};
\addplot [line width=0.72pt, white!26!black, forget plot]
table {%
1 nan
1 nan
};
\addplot [line width=0.72pt, white!26!black, forget plot]
table {%
2 nan
2 nan
};
\addplot [line width=0.72pt, white!26!black, forget plot]
table {%
0.184 nan
0.184 nan
};
\addplot [line width=0.72pt, white!26!black, forget plot]
table {%
1.184 nan
1.184 nan
};
\addplot [line width=0.72pt, white!26!black, forget plot]
table {%
2.184 nan
2.184 nan
};
\addplot [line width=0.72pt, white!26!black, forget plot]
table {%
0.368 nan
0.368 nan
};
\addplot [line width=0.72pt, white!26!black, forget plot]
table {%
1.368 nan
1.368 nan
};
\addplot [line width=0.72pt, white!26!black, forget plot]
table {%
2.368 nan
2.368 nan
};
\draw (axis cs:-0.368,1) ++(0pt,10pt) node[
  scale=0.7,
  text=black,
  rotate=0.0
]{1.00x};
\draw (axis cs:0.632,1) ++(0pt,10pt) node[
  scale=0.7,
  text=black,
  rotate=0.0
]{1.00x};
\draw (axis cs:1.632,1) ++(0pt,10pt) node[
  scale=0.7,
  text=black,
  rotate=0.0
]{1.00x};
\draw (axis cs:-0.184,1.60083499727718) ++(0pt,10pt) node[
  scale=0.7,
  text=black,
  rotate=0.0
]{1.60x};
\draw (axis cs:0.816,2.94993429697766) ++(0pt,10pt) node[
  scale=0.7,
  text=black,
  rotate=0.0
]{2.95x};
\draw (axis cs:1.816,4.29525923396506) ++(0pt,10pt) node[
  scale=0.7,
  text=black,
  rotate=0.0
]{4.30x};
\draw (axis cs:0,1.59677711388738) ++(0pt,10pt) node[
  scale=0.7,
  text=black,
  rotate=0.0
]{1.60x};
\draw (axis cs:1,2.94548317260382) ++(0pt,10pt) node[
  scale=0.7,
  text=black,
  rotate=0.0
]{2.95x};
\draw (axis cs:2,4.28100626790323) ++(0pt,10pt) node[
  scale=0.7,
  text=black,
  rotate=0.0
]{4.28x};
\draw (axis cs:0.184,1.51737783895389) ++(0pt,10pt) node[
  scale=0.7,
  text=black,
  rotate=0.0
]{1.52x};
\draw (axis cs:1.184,2.43693009118541) ++(0pt,10pt) node[
  scale=0.7,
  text=black,
  rotate=0.0
]{2.44x};
\draw (axis cs:2.184,3.1744269190326) ++(0pt,10pt) node[
  scale=0.7,
  text=black,
  rotate=0.0
]{3.17x};
\draw (axis cs:0.368,1.66176747691728) ++(0pt,10pt) node[
  scale=0.7,
  text=black,
  rotate=0.0
]{1.66x};
\draw (axis cs:1.368,3.04372584909498) ++(0pt,10pt) node[
  scale=0.7,
  text=black,
  rotate=0.0
]{3.04x};
\draw (axis cs:2.368,4.3974945375091) ++(0pt,10pt) node[
  scale=0.7,
  text=black,
  rotate=0.0
]{4.40x};
\end{axis}

\end{tikzpicture}


==> images/performance_gain.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{burlywood231187113}{RGB}{231,187,113}
\definecolor{darkgray158150204}{RGB}{158,150,204}
\definecolor{darkslategray66}{RGB}{66,66,66}
\definecolor{dimgray85}{RGB}{85,85,85}
\definecolor{gainsboro229}{RGB}{229,229,229}
\definecolor{gray119}{RGB}{119,119,119}
\definecolor{indianred2049072}{RGB}{204,90,72}
\definecolor{lightgray}{RGB}{211,211,211}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue69133171}{RGB}{69,133,171}
\definecolor{yellowgreen13817181}{RGB}{138,171,81}

\begin{axis}[
axis background/.style={fill=gainsboro229},
axis line style={white},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204,
  fill=gainsboro229
},
tick align=outside,
tick pos=left,
title={Performance Gain Across Resolutions},
unbounded coords=jump,
x grid style={lightgray},
xlabel=\textcolor{dimgray85}{Resolution},
xmajorgrids,
xmin=-0.5, xmax=2.5,
xtick style={color=dimgray85},
xtick={0,1,2},
xticklabels={1024,1536,2048},
y grid style={lightgray},
ylabel=\textcolor{dimgray85}{Performance Increase},
ymajorgrids,
ymin=0, ymax=4.59126272461832,
ytick style={color=dimgray85}
]
\draw[draw=none,fill=indianred2049072,very thin] (axis cs:-0.4,0) rectangle (axis cs:-0.266666666666667,1);
\draw[draw=none,fill=steelblue69133171,very thin] (axis cs:-0.266666666666667,0) rectangle (axis cs:-0.133333333333333,1);
\draw[draw=none,fill=darkgray158150204,very thin] (axis cs:-0.133333333333333,0) rectangle (axis cs:-5.55111512312578e-17,1.60691950148051);
\draw[draw=none,fill=gray119,very thin] (axis cs:-1.38777878078145e-17,0) rectangle (axis cs:0.133333333333333,1.88607332229864);
\draw[draw=none,fill=burlywood231187113,very thin] (axis cs:0.133333333333333,0) rectangle (axis cs:0.266666666666667,1.94219392947796);
\draw[draw=none,fill=yellowgreen13817181,very thin] (axis cs:0.266666666666667,0) rectangle (axis cs:0.4,2.11154851144224);
\draw[draw=none,fill=indianred2049072,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=indianred2049072,very thin}
\addlegendentry{Baseline (0.75)}

\draw[draw=none,fill=steelblue69133171,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=steelblue69133171,very thin}
\addlegendentry{Baseline (0.89)}

\draw[draw=none,fill=darkgray158150204,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=darkgray158150204,very thin}
\addlegendentry{ToMe (0.75)}

\draw[draw=none,fill=gray119,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=gray119,very thin}
\addlegendentry{ToMe (0.89)}

\draw[draw=none,fill=burlywood231187113,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=burlywood231187113,very thin}
\addlegendentry{ToDo (0.75)}

\draw[draw=none,fill=yellowgreen13817181,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=yellowgreen13817181,very thin}
\addlegendentry{ToDo (0.89)}

\draw[draw=none,fill=indianred2049072,very thin] (axis cs:0.6,0) rectangle (axis cs:0.733333333333333,1);
\draw[draw=none,fill=steelblue69133171,very thin] (axis cs:0.733333333333333,0) rectangle (axis cs:0.866666666666667,1);
\draw[draw=none,fill=darkgray158150204,very thin] (axis cs:0.866666666666667,0) rectangle (axis cs:1,2.41587106487414);
\draw[draw=none,fill=gray119,very thin] (axis cs:1,0) rectangle (axis cs:1.13333333333333,2.91939919507837);
\draw[draw=none,fill=burlywood231187113,very thin] (axis cs:1.13333333333333,0) rectangle (axis cs:1.26666666666667,2.92046470207517);
\draw[draw=none,fill=yellowgreen13817181,very thin] (axis cs:1.26666666666667,0) rectangle (axis cs:1.4,2.99610096552275);
\draw[draw=none,fill=indianred2049072,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\draw[draw=none,fill=steelblue69133171,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\draw[draw=none,fill=darkgray158150204,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\draw[draw=none,fill=gray119,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\draw[draw=none,fill=burlywood231187113,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\draw[draw=none,fill=yellowgreen13817181,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\draw[draw=none,fill=indianred2049072,very thin] (axis cs:1.6,0) rectangle (axis cs:1.73333333333333,1);
\draw[draw=none,fill=steelblue69133171,very thin] (axis cs:1.73333333333333,0) rectangle (axis cs:1.86666666666667,1);
\draw[draw=none,fill=darkgray158150204,very thin] (axis cs:1.86666666666667,0) rectangle (axis cs:2,3.14346727181141);
\draw[draw=none,fill=gray119,very thin] (axis cs:2,0) rectangle (axis cs:2.13333333333333,4.27562459437732);
\draw[draw=none,fill=burlywood231187113,very thin] (axis cs:2.13333333333333,0) rectangle (axis cs:2.26666666666667,4.27627976887371);
\draw[draw=none,fill=yellowgreen13817181,very thin] (axis cs:2.26666666666667,0) rectangle (axis cs:2.4,4.37263116630317);
\draw[draw=none,fill=indianred2049072,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\draw[draw=none,fill=steelblue69133171,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\draw[draw=none,fill=darkgray158150204,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\draw[draw=none,fill=gray119,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\draw[draw=none,fill=burlywood231187113,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\draw[draw=none,fill=yellowgreen13817181,very thin] (axis cs:0,0) rectangle (axis cs:0,0);
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
-0.333333333333333 nan
-0.333333333333333 nan
};
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
-0.2 nan
-0.2 nan
};
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
-0.0666666666666667 nan
-0.0666666666666667 nan
};
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
0.0666666666666667 nan
0.0666666666666667 nan
};
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
0.2 nan
0.2 nan
};
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
0.333333333333333 nan
0.333333333333333 nan
};
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
0.666666666666667 nan
0.666666666666667 nan
};
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
0.8 nan
0.8 nan
};
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
0.933333333333333 nan
0.933333333333333 nan
};
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
1.06666666666667 nan
1.06666666666667 nan
};
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
1.2 nan
1.2 nan
};
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
1.33333333333333 nan
1.33333333333333 nan
};
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
1.66666666666667 nan
1.66666666666667 nan
};
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
1.8 nan
1.8 nan
};
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
1.93333333333333 nan
1.93333333333333 nan
};
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
2.06666666666667 nan
2.06666666666667 nan
};
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
2.2 nan
2.2 nan
};
\addplot [line width=0.9pt, darkslategray66, forget plot]
table {%
2.33333333333333 nan
2.33333333333333 nan
};
\draw (axis cs:-0.333333333333333,1) ++(0pt,3pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{1.00x};
\draw (axis cs:-0.2,1) ++(0pt,3pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{1.00x};
\draw (axis cs:-0.0666666666666667,1.60691950148051) ++(0pt,5pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{1.61x};
\draw (axis cs:0.0666666666666666,1.88607332229864) ++(0pt,2pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{1.89x};
\draw (axis cs:0.2,1.94219392947796) ++(0pt,10pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{1.94x};
\draw (axis cs:0.333333333333333,2.11154851144224) ++(0pt,10pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{2.11x};
\draw (axis cs:0.666666666666667,1) ++(0pt,5pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{1.00x};
\draw (axis cs:0.8,1) ++(0pt,5pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{1.00x};
\draw (axis cs:0.933333333333333,2.41587106487414) ++(0pt,10pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{2.42x};
\draw (axis cs:1.06666666666667,2.91939919507837) ++(0pt,10pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{2.92x};
\draw (axis cs:1.2,2.92046470207517) ++(0pt,10pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{2.92x};
\draw (axis cs:1.33333333333333,2.99610096552275) ++(0pt,10pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{3.00x};
\draw (axis cs:1.66666666666667,1) ++(0pt,5pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{1.00x};
\draw (axis cs:1.8,1) ++(0pt,5pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{1.00x};
\draw (axis cs:1.93333333333333,3.14346727181141) ++(0pt,10pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{3.14x};
\draw (axis cs:2.06666666666667,4.27562459437732) ++(0pt,0pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{4.28x};
\draw (axis cs:2.2,4.27627976887371) ++(0pt,10pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{4.28x};
\draw (axis cs:2.33333333333333,4.37263116630317) ++(0pt,10pt) node[
  scale=0.5,
  text=black,
  rotate=0.0
]{4.37x};
\end{axis}

\end{tikzpicture}

